Simulating the Galactic population of axion clouds around stellar-origin black holes: Gravitational wave signals in the 10-100 kHz band

Ultralight scalar fields can experience runaway `superradiant' amplification near spinning black holes, resulting in a macroscopic `axion cloud' which slowly dissipates via continuous monochromatic gravitational waves. For a particular range of boson masses, $\mathcal{O}(10^{-11}$ -- $10^{-10})$ eV, an axion cloud will radiate in the $10$ -- $100$ kHz band of the Levitated Sensor Detector (LSD). Using fiducial models of the mass, spin, and age distributions of stellar-origin black holes, we simulate the present-day Milky Way population of these hypothetical objects. As a first step towards assessing the LSD's sensitivity to the resultant ensemble of GW signals, we compute the corresponding signal-to-noise ratios which build up over a nominal integration time of $10^{7}$ s, assuming the projected sensitivity of the $1$-m LSD prototype currently under construction, as well as for future $10$-m and $100$-m concepts. For a $100$-m cryogenic instrument, hundreds of resolvable signals could be expected if the boson mass $\mu$ is around $3\times10^{-11}$ eV, and this number diminishes with increasing $\mu$ up to $\approx 5.5\times10^{-11}$ eV. The much larger population of unresolved sources will produce a confusion foreground which could be detectable by a $10$-m instrument if $\mu \in (3-4.5)\times10^{-11}$ eV, or by a $100$-m instrument if $\mu \in (3-6)\times10^{-11}$ eV.

==> Sections/Commented_out_text.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%COMMENTED-OUT TEXT

%ABSTRACT
%Our simulations indicate the foreground does not rise sufficiently above the $1$-m detector's noise floor to achieve detection, and it remains for future work to assess the capabilities of a network of $1$-m detectors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.5\textwidth]{Images/galaxyfracs.png}
%    \caption{Fractions of axion clouds $f_{i} = N_{i}/N_{tot}$ in the three Galactic regions, $i = (\text{thin disk},\ \text{thick disk},\ \text{bulge})$. The hierarchy of cloud fractions is determined by the complex interplay between cloud growth timescales, GW dissipation timescales, and source distance (which determines the GW propagation time).} 
%    \label{fig:galaxyfracs}
%\end{figure}
%\begin{figure*}
%    \centering
%    \includegraphics[width=0.5\textwidth]{Images/timescales3.png}
%    \caption{The distribution of axion cloud growth timescales $\tau_{c}$ and dissipation timescales $\tau_{\text{GW}}$ for $\mu = 3\cross10^{-11}$ eV.} 
%    \label{fig:timescales3}
%\end{figure*}
%\begin{figure*}
%    \centering
%    \includegraphics[width=0.5\textwidth]{Images/mcloud3.png}
%    \caption{The distribution of axion cloud masses $M_{c}$ for $\mu = 3\cross10^{-11}$ eV. The mean mass is $0.3\ M_{\odot}$, the standard deviation is $0.1\ M_{\odot}$, the mode is $0.25\ M_{\odot}$, and the most massive cloud in the population has $M_{c} = 0.82\ M_{\odot}$.} 
%    \label{fig:mcloud3}
%\end{figure*}

%\begin{figure*}
%    \centering
%    \includegraphics[width=0.6\textwidth]{Images/fcbh0.png}
%    \caption{The source-frame GW frequencies $f_{\text{GW,s}}$ and initial BH spins $\chi_{i}$ for the extant clouds in the $3\times 10^{-11}$ eV simulation.} 
%    \label{fig:}
%\end{figure*}


%SECTION VI.A.
%\indent In Sec$.$ III, we noted that the GW emission from axion clouds can be computed in the fully-classical Teukolsky formalism. This might be surprising since ultralight scalars are a topic usually discussed in a quantum field theory context. However, axion clouds are macroscopic objects amenable to a classical analysis. In all of our simulated populations, the average cloud mass is around $0.3\ M_{\odot}$ (with standard deviations $\mathcal{O}(0.01 - 0.1)\ M_{\odot}$), with the most massive clouds reaching $\approx0.8\ M_{\odot}$ (Fig$.$ \ref{fig:mcloud3}). Such objects carry the mass of a small star, so they are best described in the macroscopic formalism of a classical field propagating on a curved background.  \\ \\
%\indent Generally, the Galactic thin disk hosts around $50\%$ of all axion clouds, while the thick disk hosts around $20\%$ (Fig$.$ \ref{fig:galaxyfracs}).   \\ \\


%\begin{figure*}
%	\includegraphics[width=1.0\textwidth]{Images/xir8.png}
%	\caption{The real part of the $n = 8$ bound-state eigenfrequency. As $\alpha \rightarrow 0$, $\xi_{R} \rightarrow 1$, and $\omega_{R} \rightarrow \mu / \hbar$. Since $\omega_{GW} = 2\omega_{R}$, the GW frequency depends only on the axion mass in the $\alpha \ll 1$ limit.}
%	\label{fig:xir8}
%\end{figure*}



